Routing for Intermittently-Powered Sensing Systems

Recently, intermittent computing (IC) has received tremendous attention due to its high potential in perpetual sensing for Internet-of-Things (IoT). By harvesting ambient energy, battery-free devices can perform sensing intermittently without maintenance, thus significantly improving IoT sustainability. To build a practical intermittently-powered sensing system, efficient routing across battery-free devices for data delivery is essential. However, the intermittency of these devices brings new challenges, rendering existing routing protocols inapplicable. In this paper, we propose RICS, the first-of-its-kind routing scheme tailored for intermittently-powered sensing systems. RICS features two major designs, with the goal of achieving low-latency data delivery on a network built with battery-free devices. First, RICS incorporates a fast topology construction protocol for each IC node to establish a path towards the sink node with the least hop count. Second, RICS employs a low-latency message forwarding protocol, which incorporates an efficient synchronization mechanism and a novel technique called pendulum-sync to avoid the time-consuming repeated node synchronization. Our evaluation based on an implementation in OMNeT++ and comprehensive experiments with varying system settings show that RICS can achieve orders of magnitude latency reduction in data delivery compared with the baselines.

==> 1-introduction-gs.tex <==
\section{Introduction}
Intermittent computing (IC) has received increasing traction recently considering its high potential in sustainable Internet-of-Things (IoT) applications~\cite{2017-snapl-survey,2020-asplos-chrt,2020-asplos-tics,2020-imwut-bfgame,2020-imwut-bfree,2022-mobisys-bluetooth,2022-pldi-wario,2021-csur-sync}.
\lin{Former works focus on keeping the system consistent or synchronizing between two IC nodes.
The state-of-art work can make IC nodes with tiny capacitors charge and discharge quickly as if the system can work constantly without interruptions. Whereas, the small working overlap between those devices makes stable communication between any pairwise nodes difficult. The state-of-art work (Find~\cite{2021-nsdi-find}, Bonito~\cite{2022-nsdi-bonito}) uses probability methods with delayed working intervals to make IC nodes discover each other. They solve the synchronization scenarios in homogeneous charging time and heterogeneous charging time respectively.}
\begin{mysout}
IC relies on \emph{battery-free} low-power devices, which harvest ambient energy from the environment (e.g., light, radio-frequency signals, and kinetic energy) and accumulate the energy in capacitors to function~\cite{2020-imwut-bfgame,2017-imwut-bfphone}. 
These devices require zero maintenance once deployed and are environment-friendly attributed to the absence of batteries which typically contain hazardous chemicals. 
Recently, rapid hardware advances in low-power micro-controller units (MCUs), non-volatile memories, efficient energy-harvesting units, and tiny capacitors have laid a solid foundation for IC~\cite{2018-asplos-energystore,2017-snapl-survey,2021-nsdi-find}. 
% Meanwhile, the cost of IC devices has also decreased considerably. 
Driven by such development, researchers have explored the feasibility of leveraging IC in various pervasive application domains, especially in fierce and unmanned environments.  
For example, IC has been employed to build sensing systems for monitoring the atmosphere, forests, and oceans~\cite{2020-sensys-bfsensing,2021-weee-cic,2022-tecs-camaroptera,2022-nc-underwater}, where some of them are even equipped with machine learning inference~\cite{2019-asplos-genesis}.
\end{mysout}

\begin{mysout}
However, the intermittent nature of IC devices brings challenges to building such sensing systems. 
Typically, a sensing system consists of a large number of dispersed nodes, which collect data from the environment and send the data to a common, more powerful sink node for complex processing. 
Since not all nodes can communicate with the sink directly (due to limited radio coverage of the IC device), data has to be \emph{routed} across the nodes.
\end{mysout}
\lin{However, multiple communication scenarios have been explored so far. 
To make it practical, typically, IC nodes need to collect data and route hop-by-hop to a more powerful sink node like the scenario in traditional WSNs in the scenario~\cite{2018-trustCom-ESRQ}. 
Here, we summarize the following two general challenges that arise compared with traditional WSNs and DTNs~\cite{2009-ICST-DTNs}: }
(1) IC nodes need to form a network and each IC node needs to acquire routing information for reaching the sink. 
Such topological information cannot be set in advance since the node distribution can be quite random during the system deployment.
In traditional sensor networks, battery-powered nodes calculate their locations with the aid of auxiliary components like GPS units, which are too power-consuming for IC devices.
(2) Based on the acquired routing information, an IC node has to be synchronized, with respect to the working time (during which the IC device is active), with its next-hop IC node specified in the routing information. 
\lin{This is critical for ensuring successful data transfer since the working time of different IC nodes is likely different. 
Being a complex task per se, such synchronization has to happen on a per-message, per-hop basis, leading to an extremely time-consuming process and energy consumption (more than $1000 \times$)~\cite{2022-nsdi-bonito} that can greatly degrade the routing performance, leading to large data delivery delays.
\emph{Therefore, efficient routing is key to building a practical sensing system with IC devices.}}

% Since not all nodes can communicate with the sink directly (due to limited radio coverage of the IC device), data has to be \emph{routed} across the nodes. 


% However, the intermittent nature of IC devices brings challenges to building such sensing systems. 
% Typically, a sensing system consists of a large number of dispersed nodes, which collect data from the environment and send the data to a common, more powerful sink node for complex processing. 
% Since not all nodes can communicate with the sink directly (due to limited radio coverage of the IC device), data has to be \emph{routed} across the nodes. 
% The following two challenges arise: 
% (1) IC nodes need to form a network and each IC node needs to acquire routing information for reaching the sink. 
% Such topological information cannot be set in advance since the node distribution can be quite random during the system deployment.
% In traditional sensor networks, battery-powered nodes calculate their locations with the aid of auxiliary components like GPS units, which are too power-consuming for IC devices.
% (2) Based on the acquired routing information, an IC node has to be synchronized, with respect to the working time (during which the IC device is active), with its next-hop IC node specified in the routing information. 
% This is critical for ensuring successful data transfer, since the working time of different IC nodes is likely different. 
% Being a complex task per se, such synchronization has to happen on a per-message, per-hop basis, leading to an extremely time-consuming process that can greatly degrade the routing performance, leading to large data delivery delays.
% \emph{Therefore, efficient routing is key to building a practical sensing system with IC devices.}

\begin{mysout}
Existing efforts fall short of addressing the routing problem in intermittently-powered sensing systems. 
On the IC research front, there have been works on exploring the communication issue between a pair of IC devices~\cite{2021-mass-comm,2021-nsdi-find,2022-nsdi-bonito}. 
However, the main focus, so far, is on working time synchronization, which is a major challenge in IC environments~\cite{2021-csur-sync}. 
For example, Find builds a delay model based on a geometric distribution for improving the encountering probability of the working time of two IC devices to facilitate synchronization~\cite{2021-nsdi-find}. 
Recently, a Bluetooth Low Energy (BLE) implementation has been presented for IC devices without protocol specification changes~\cite{2022-mobisys-bluetooth}.
While we will build on these steps, these works do not address the problem of multi-hop routing across a set of IC devices.
Meanwhile, existing routing protocols for traditional wireless sensor networks, as well as for energy-harvesting wireless sensor networks that harvest energy to recharge sensor batteries, are ill-suited for IC devices since they typically assume more capable nodes (e.g., powered by batteries), often also equipped with geo-location devices, which allow for complex routing protocols to be implemented~\cite{2012-csur-wsn,2018-tsn-ehwsn}. 
Also, due to the absence of intermittency, these protocols do not account for the working time synchronization overhead, which is critical to the performance of sensing systems with IC devices. 
\emph{To the best of our knowledge, none of the existing works can fully address the routing problem in intermittently-powered sensing systems.}
\end{mysout}{}

In this paper, we propose a new routing scheme called \namex, tailored for \underline{R}outing in \underline{IC} \underline{S}ensing systems. 
\lin{Routing performance is affected by different application scenarios and energy harvesting efficiency. \namex does not pursue a general solution to solve all routing problems in different scenarios.  
\namex focuses on the routing challenges when the IC nodes have the similar or same charging times as the scenarios in \emph{Find}, more discussions will do in Section~\ref{sec:design} and Section~\ref{sec:discussion}. 
More complex scenarios will be explored in our future work.}
The goal of \namex is to ensure efficient data transfer across IC nodes so that the data (e.g., sensor readings) generated by each IC node can be delivered to the sink node as timely as possible. 
\namex achieves this goal by featuring the following two specific designs.
First, we propose an \emph{efficient topology construction} protocol where each IC node decides its best next hop for passing messages toward the sink node.
Our proposed protocol starts from the sink node and disseminates and updates the minimum hop count of each node to the sink iteratively. 
Our protocol ensures finding the path for each node to reach the sink node with the least hop count, minimizing the data delivery delay. 
\lin{Second, we propose a \emph{low-latency message forwarding} protocol based on a technique called pendulum-sync that allows the IC node to swing forth its working time (based on the cached offset) to match with its next hop for communication and swing back when the communication is completed.}
With such a protocol, \namex eliminates the need for frequent working time synchronization among the IC nodes, thus reducing the delay in message forwarding and data delivery significantly.

\begin{mysout}
Second, we propose a \emph{low-latency message forwarding} protocol based on a technique called pendulum-sync. 
Given a path from an IC node to the sink produced in topology construction, each of the nodes on the path has to synchronize its working time with its next hop before its communication can start. 
This leads to significant time overhead in data delivery if such synchronization is required for each individual message along the path. 
We observe that the offset between the working time of neighboring IC nodes on the path is static and, thus, the IC node can cache the offset to avoid the expensive repeated synchronization. 
We propose pendulum-sync, a technique that allows the IC node to swing forth its working time (based on the cached offset) to match with its next hop for communication and swing back when the communication is completed. 
With such a protocol, \namex eliminates the need for frequent working time synchronization among the IC nodes, thus reducing the delay in message forwarding and data delivery significantly.
\end{mysout}

Overall, we make the following contributions to this paper:
\begin{enumerate}[label=(\arabic*)]
    \item  \sout{We identify the key challenges for efficient routing in intermittently-powered sensing systems (Section~\ref{sec:motivation}) and propose the first routing scheme \namex to address them.}
    \item We propose an efficient topology construction protocol (Section~\ref{sec:topology}) for building the least-hop path for each IC node to the sink node given a set of IC nodes.
    \item We propose a low-latency message forwarding protocol (Section~\ref{sec:routing}) based on a new technique called pendulum-sync, which caches the working time offset between IC nodes and dynamically adapts the working time of each IC node to communicate with its next hop.
    \item We implement \namex in OMNeT++ and perform extensive experiments to validate its performance under various scenarios and settings (Section~\ref{sec:evaluation}). Our results show that \namex achieves orders of magnitude reduction in the data delivery latency compared with the baselines.
\end{enumerate}
\lin{
Section~\ref{sec:design} gives the overall design of \namex.
Section~\ref{sec:discussion} discusses the limitations of \namex. Section~\ref{sec:conclusions} draws the conclusions and our future works.
}
% Section~\ref{sec:discussion} discusses the limitations of \namex. Section~\ref{sec:relatedwork} summarizes related works. Section~\ref{sec:conclusions} draws the conclusions.

==> 2-motivation.tex <==
\section{Background and Motivation}
\label{sec:motivation}

We provide a brief introduction to intermittent computing and summarize works on routing in wireless sensor networks, from which we motivate our work. We also identify the challenges for routing in intermittently-powered sensing systems.

\subsection{Intermittent Computing}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.48\textwidth,page=1]{figures/figures.pdf}
%     \caption{An IC device alternates between the charging (off) and the working (on) mode. A charging cycle consists of one charging period and one working period.}
%     \label{fig:ic-process}
% \end{figure}

Intermittent computing (IC) employs battery-free devices that harvest energy from the ambient environment and store the collected energy in \emph{capacitors} to power on the device intermittently~\cite{2017-snapl-survey}. 
The IC device enters the working mode (powered on) to perform computations and/or communications when the stored energy on the capacitor reaches an upper threshold $E_{ON}$. 
The IC device falls into the charging mode (powered off) to charge the capacitor when the stored energy drops below a lower threshold $E_{OFF}$. 
Charging the capacitor takes time and the capacitor has limited space for energy storage. 
Therefore, the IC device alternates between the working and charging modes.
A \emph{charging cycle} is defined as the continuous time period from when the IC device enters the charging mode until it exists in the working mode.
Typically, IC devices can only maintain their working mode for a very short period of time (e.g., a few milliseconds or less~\cite{2021-nsdi-find}).
This characteristic imposes multiple challenges for both computing and communication with IC devices. 

\subsubsection{Computing on IC devices} 
Since the working period of the IC device is short, it is unlikely that a sophisticated program can finish its execution within a single charging cycle of the IC device. 
Hence, the execution of the program will have to span multiple charging cycles, with the device alternating between charging and working modes.
For the program to make forward progress, the program state has to be preserved before every power failure. 
This way, the program can continue its execution with the preserved state when the IC device powers on again.
IC devices are typical with non-volatile memories like FRAM~\cite{2022-pldi-wario} for saving the state during power failures.
In addition, repeated power failures may leave the memory inconsistent due to partial or repeated updates to the non-volatile memory. 
This problem has been extensively studied recently and existing solutions can be generally divided into two categories: 
(1) \emph{Checkpoint-based} approaches insert checkpoints into the program manually or through compiler analysis, and the runtime system makes copies for the processor state on these checkpoints during the program execution~\cite{2019-pldi-samoyed,2020-tecs-checkpoint,2022-pldi-wario}. 
(2) \emph{Task-based} approaches transform the program into tasks which, upon a power failure, are re-executed after recovery~\cite{2016-oopsla-chain,2019-asplos-genesis,2017-oopsla-alpaca}. Memory consistency is guaranteed by ensuring that the partial execution of a task is not visible to a subsequent re-execution. 
These works, while focusing on a single IC device, have laid a solid foundation for the adoption of IC devices in sensing systems.

\subsubsection{Communication between IC devices} 
Due to the intermittency brought by frequent power failures, it is not guaranteed that two IC devices will be powered on at the same time so that they can discover and communicate with each other. 
Since the working time of an IC device is rather short (typically at the level of a few milliseconds or less) in each charging cycle, synchronizing the working time of two IC devices is crucial for successful communication between them. 
The most representative works addressing this issue are Find~\cite{2021-nsdi-find} and Bonito~\cite{2022-nsdi-bonito}. 
Recently, a Bluetooth Low Energy (BLE) implementation for IC devices has been presented, allowing IC devices to communicate with BLE without changes to the protocol specification~\cite{2022-mobisys-bluetooth}.
So far, existing works are mainly focused on the communication between a pair of IC devices; no work has been done on multi-hop routing in a large network of IC devices. 

\subsection{Routing in Wireless Sensor Networks}

Wireless sensor networks (WSNs) rely on battery-powered embedded devices to form a network for sensing applications. 
As a core functionality, routing in WSNs has been extensively explored, optimizing different quality of service (QoS) metrics including latency and node energy balance~\cite{2012-csur-wsn}. 
Among them, a variety of cluster-based and opportunistic routing protocols have been proposed~\cite{2012-csur-wsn}. 
Unfortunately, none of these protocols are directly applicable to intermittently-powered sensing systems since they do not account for intermittency which barely exists in traditional  battery-powered WSNs. 
Moreover, nodes in a WSN are typically more capable than IC devices powered on harvested energy stored in a capacitor, allowing relatively more complex routing protocols to be executed, e.g., leveraging extra geo-location devices. 
Some works have also explored energy-harvesting WSNs where energy-harvesting devices are used to recharge on-board batteries~\cite{2018-tsn-ehwsn}. 
Being aware of the availability of harvested energy, the routing protocols for energy-harvesting WSNs make similar assumptions on the capability of WSN nodes and, thus, are inapplicable for intermittently-powered sensing systems. 

\subsection{Routing in Intermittently-Powered Sensing Systems}
%重点突出此路由协议是在理想的条件下设计的 (强假设). 是对间歇条件下路由的探索, 为后来的复杂条件下路由奠定基础. 

Based on the above analysis, we argue that new routing protocols are required for intermittently-powered sensing systems, which have not been explored so far. 
Our goal is to make the first attempt at dissecting the routing problem and exploring the design space under reasonable assumptions (detailed in Section~\ref{sec:design}) for the sake of tractability.  
We note that the routing problem is non-trivial even under our simplified scenarios. 
In particular, we identify the following two challenges brought by the intermittency of IC devices: 
(1) \emph{Topology construction} where each IC node in an intermittently-powered sensing system has to determine the best path (i.e., with the least hop count) to the sink node. 
The challenge is to construct such information across all IC nodes without central coordination, with their working time unknown to each other.
To this end, we provide an efficient topology construction protocol, which we detail in Section~\ref{sec:topology}. 
(2) \emph{Message forwarding} where IC nodes on a routing path generated in the topology construction process can forward messages towards the sink efficiently without incurring large latency overhead for repeated working time synchronization between neighboring nodes on every hop on the path. 
We provide a low-latency message forwarding protocol to address this issue, which is detailed in Section~\ref{sec:routing}.

==> 8-relatedwork.tex <==
\section{Related work}
\label{sec:relatedwork}

In this section, we summarize related works in two parts. 
% focusing on communication between IC devices and in energy-harvesting WSNs. 
First, we present works that study the communication between two battery-free nodes. 
Then, we discuss works on the routing in energy-harvesting WSNs.

\subsection{Communication Between Two IC Devices} 
One-to-end communication between battery-free devices is a well-recognized issue. 
To address the challenges brought by intermittency.
Recently, a lot of work has been done on the communication issue between two battery-free devices. 
To reduce latency and improve efficiency, Rajib and Nasipuri propose a method for achieving transmission diversity by adopting cooperative relaying and opportunistic routing with the help of neighboring nodes~\cite{2018-tecs-predic}. 
They also employ a predictive retransmission strategy to improve the retransmission success rate.
Deep et al. propose the concept of lifecycle management protocol (LMP)---a stateless communication framework based on selecting a random wake-up time for the two nodes and upon overlap extending the working time of the two nodes to maximize communication opportunity. 
They provide theoretical analysis for their approach and evaluate it on a prototype.
Find aims to synchronize the working time of two IC nodes for communication with a random delay scheme where it is shown that a random delay drawn from a geometric distribution provides the lowest discovery latency~\cite{2021-nsdi-find}. 
Bonito allows IC nodes to learn a charging distribution online and leverages the learned information to adapt the working time of IC nodes to maximize communication opportunity~\cite{2022-nsdi-bonito}.
While building a solid foundation for communication between IC devices, these works are focused on a single link between two IC devices, thus not applicable to the routing problem we study in this paper.


% Find~\cite{2021-nsdi-find} uses the random delay scheme complied with geometric distribution to synchronize the overlapping intervals between two BNs. In Find, it assumes every node has the same charging time and works in the same energy condition. Furthermore, Bonito~\cite{2022-nsdi-bonito} is an extended work of Find. Bonito can sustain a long consistent communication period between two BNs after their first encounter by exchanging delay model parameters.  Similarly,  a work based on the prediction re-transmission mechanism decreases the routing delay by using a probabilistic delay model in energy-harvested WSNs~\cite{2018-tecs-predic}. Moreover,
% Lifecycle management protocol (LMP)~\cite{2021-mass-comm} is a stateless communication scheme to extend interval time between two batteryless nodes. Initially, those nodes select a random work-on interval time.  Batteryless nodes extend their work-on period to maximize the communication time when they detect overlapping. However, the LMP does not do any synchronization operations.  In addition, LMP allows batteryless nodes to transmit and listen to data multi times. To summarize, those works can not be applied in the routing in intermittently powered networks because they focus on solving communication problems between two batteryless nodes.

\subsection{Routing in Energy-Harvesting WSNs}
Energy-harvesting WSNs have been well studied with many routing schemes proposed~\cite{2018-tsn-ehwsn}.
For example, ESC is a protocol for synchronizing the energy supply with demand to optimize reliable data transmissions in energy-harvested WSNs~\cite{2009-icnp-esc}. 
While using a similar cyclic working time schedule, ESC does not rely on synchronization operations since it assumes a long working period during which communication can happen without working time synchronization. 
Negishi et al. propose an opportunistic routing protocol for energy-harvesting WSNs with pre-assigned coordination~\cite{2014-apcc-ehwsn}. 
Similarly, they assume that nodes have long working periods. 
In a nutshell, all these existing works do not work for IC devices that have a working period at the scale of milliseconds or even microseconds.


% An opportunistic routing mechanism for batteryless networks based on pre-assigned coordination was proposed~\cite{2014-apcc-ehwsn}, which routes based on the probabilistic relying mode by referring the distance between receivers and senders. However, it assumes nodes can work for a long period, it does not comply with intermittently powered network conditions (work in $ms$ or $us$ scale).
% ESC~\cite{2009-icnp-esc} presents the first cyclic work schedule in EHWSNs. ESC denotes the batteryless nodes’ work schedule by a circle with multiple work-on slots to increase the probability of encounters. However, ESC does not do synchronization operations, and hypothesis nodes have long work-on periods and know each other's coordination information. In summary, state-of-art work cannot solve routing problems in intermittently powered networks because they do not have special support to IC nodes.

% \textbf{Communication between two batteryless nodes:}
% Find~\cite{2021-nsdi-find} uses the random delay scheme complied with geometric distribution to synchronize the overlapping intervals between two BNs. In Find, it assumes every node has the same charging time and wrok in the same energy condition. Moreover,  a proposed work based on the prediction re-transmission mechanism to decrease the routing delay by using a probabilistic delay model in energy-harvested WSNs~\cite{2018-tecs-predic}. Bonito~\cite{2022-nsdi-bonito} is an extended work of Find. Bonito can sustain a long consistent communication period between two BNs after their first encounter by exchanging delay model parameters.  Lifecycle management protocol (LMP)~\cite{2021-mass-comm} is a stateless communication scheme to extend interval time between two batteryless nodes. Initially, those nodes select a random working interval time.  Batteryless nodes extend their working period to maximise the communication time when they detect overlapping. However, the LMP does not do any synchronization operations.  In addition, LMP allows IC  nodes to transmit and listen to data multi times. However, those works can not be applied in the routing because they focus on solving problems between two IC nodes or non-synchronization problems.

% \textbf{Communication in batteryless sensor networks:}
% CIS~\cite{2020-ipsn-cis} is the first ICS cooperation mechanism.  IC nodes broadcast their wake-up information to their neighbours before their next power cycles.  Neighbouring IC nodes’  spread their wake-up times uniformly by using a randomization delay model. Therefore, IC nodes work alternatively and sequentially with the help of CIS and the whole CIS works like continuously. ESC~\cite{2009-icnp-esc} presents the first cyclic working schedule in EHWSNs.  ESC denotes the batteryless nodes’ working schedule by a circle for encountering the next hop wake-up slot before transmission. Moreover,  batteryless nodes have multiple working slots in a working cycle. The delay synchronization model can not be applied in IC nodes directly because it allows the batteryless nodes to change their duty cycles by increasing wake-up time. ReNEW~\cite{2021-tgcn-renew} attempts to improve the reliability and decrease the latency of Energy-harvested wireless sensor networks by optimising the energy distribution model.
% besides,An opportunistic routing mechanism for batteryless networks based on pre-assigned coordination was proposed~\cite{2014-apcc-ehwsn}, which decides routing slots based on the distance between receivers and senders, and the corresponding probabilistic relying model. However, they do not do synchronization operations and hypothesis nodes can work for a long time and know each other's coordination information.


==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

